OV-DINO: Unified Open-Vocabulary Detection with Language-Aware Selective Fusion

Open-vocabulary detection is a challenging task due to the requirement of detecting objects based on class names, including those not encountered during training. Existing methods have shown strong zero-shot detection capabilities through pre-training and pseudo-labeling on diverse large-scale datasets. However, these approaches encounter two main challenges: (i) how to effectively eliminate data noise from pseudo-labeling, and (ii) how to efficiently leverage the language-aware capability for region-level cross-modality fusion and alignment. To address these challenges, we propose a novel unified open-vocabulary detection method called OV-DINO, which is pre-trained on diverse large-scale datasets with language-aware selective fusion in a unified framework. Specifically, we introduce a Unified Data Integration (UniDI) pipeline to enable end-to-end training and eliminate noise from pseudo-label generation by unifying different data sources into detection-centric data format. In addition, we propose a Language-Aware Selective Fusion (LASF) module to enhance the cross-modality alignment through a language-aware query selection and fusion process. We evaluate the performance of the proposed OV-DINO on popular open-vocabulary detection benchmarks, achieving state-of-the-art results with an AP of 50.6% on the COCO benchmark and 40.1% on the LVIS benchmark in a zero-shot manner, demonstrating its strong generalization ability. Furthermore, the fine-tuned OV-DINO on COCO achieves 58.4% AP, outperforming many existing methods with the same backbone. The code for OV-DINO is available at https://github.com/wanghao9610/OV-DINO.

==> texs/11_acknowledge.tex <==
\section*{Acknowledgments}
This should be a simple paragraph before the References to thank those individuals and institutions who have supported your work on this article.

==> texs/13_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/hao_wang.jpg}}]{Hao Wang}
received the B.E. degree from Beijing Jiaotong University in 2015 and the M.S. degree from the Chinese Academy of Sciences in 2019, respectively. He is currently working toward a Ph.D degree in the Human Cyber Physical Intelligence Integration Lab, at Sun Yat-sen University, Shenzhen, China. His current research interests include deep learning on multimodal learning and open-scene understanding.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/pengzhen_ren.jpg}}]{Pengzhen Ren} is currently conducting postdoctoral research at the School of Intelligent Engineering, Sun Yat-sen University. He received his Ph.D. in Software Engineering from Northwestern University in China in 2022. He has published many papers in top AI conferences and journals such as CVPR, ICLR, AAAI, IJCAI, TPAMI, and TNNLS. Currently, he mainly focuses on the fields of vision-language pre-training, segmentation, multimodal learning, and visual self-supervision.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/zequn_jie.jpg}}]{Zequn Jie} received the B.E. degree in 2012 from the University of Science and Technology of China, Hefei, China, and the Ph.D. degree in 2016 from the National University of Singapore, Singapore. He was a Post-Doctoral Research Fellow with the Department of Electrical and Computer Engineering, National University of Singapore. He is currently a researcher in Meituan Inc., leading a team focusing on multi-modal LLM and 2D/3D perception. Prior to coming to Meituan, he was a senior researcher at Tencent AI Lab. His research interests mainly fall in the fundamental computer vision topics, e.g. supervised and weakly-supervised object detection, localization and semantic segmentation. He regularly serves as a reviewer of several top-tier conferences and journals, e.g. CVPR, ICCV, ECCV, NeurIPS, ICML, TPAMI.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/xiao_dong.jpg}}]{Xiao Dong} is currently a Ph.D. candidate of the School of Artificial Intelligence at Sun Yat-Sen University. His research interests include multi-modal retrieval and cross-modal pretraining.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/chengjian_feng.jpeg}}]{Chengjian Feng} is currently a researcher at Meituan, Shenzhen, China. He received his B.E. degree from Guangdong University of Technology of China in 2020. His research focuses on object detection, automatic driving, visual language models, and multi-modal large language models. He regularly serves as a reviewer of top AI conferences such as CVPR, ICCV, ECCV, and NeurIPS.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/yinlong_qian.jpg}}]{Yinlong Qian} is currently a researcher in Meituan, Beijing, China. He received his B.E. and Ph.D. degrees from University of Science and Technology of China in 2011 and 2017, respectively. He is currently a researcher in Meituan, Beijing, China.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/lin_ma.jpg}}]{Lin Ma} is now a Researcher with Meituan, Beijing, China. Previously, he was a Principal Researcher with Tencent AI Lab, Shenzhen, China from Sept. 2016 to Jun. 2020. He was a Researcher with Huawei Noah's Ark Lab, Hong Kong from Aug. 2013 to Sept. 2016. He was a Research Assistant with the Department of Electronic Engineering, CUHK, from Nov. 2008 to Jul. 2009. He received his Ph.D. degree in Department of Electronic Engineering at the Chinese University of Hong Kong (CUHK) in 2013. He received the B. E., and M. E. degrees from Harbin Institute of Technology, Harbin, China, in 2006 and 2008, respectively, both in computer science. He was a Visiting Student at the School of Computer Engineering, Nanyang Technological University (NTU), from Jul. 2011 to Sept. 2011. He was a Research Intern in Microsoft Research Asia from Oct. 2007 to Mar. 2008. He was a finalist to HKIS young scientist award in engineering science in 2012. He was awarded the Microsoft Research Asia fellowship in 2011. He got the best paper award in Pacific-Rim Conference on Multimedia (PCM) 2008.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/dongmei_jiang.jpg}}]{Dongmei Jiang} received her PhD degree in Computer Science and Technology from the Northwestern Polytechnical University (NPU), Xi'an China in 2000. From 2000 to 2022, she was affiliated with NPU where she became a professor in 2010. In 2023, she moved to the Peng Cheng Laboratory as a principal scientist. Her research topic has been focused on multimodal fundamental models and multimodal affective computing, on which she has published around 100 papers. She has been the local chair of ACII2015 and BigMM2018, publication co-chair of ACII2017 to ACII2021 and ACII2023, and publicity co-chair of ICMI2021.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/yaowei_wang.jpg}}]{Yaowei Wang}(Member, IEEE) is currently a professor with the Peng Cheng Laboratory and Harbin Institute of Technology, Shenzhen. He is a recipient of the special government allowances of the State Council. He is the author or co-author of more than 140 technical articles in international journals and conferences, including TPAMI, ACM MM, IEEE TIP, and CVPR. His current research interests include multimedia content analysis and understanding, machine learning, and computer vision. He serves as the chair of the IEEE Digital Retina Systems Working Group and a member of IEEE, CIE, CCF, CSIG. He was the recipient of the second prize of the State Technological Invention Award in 2017, the first prize of the CIE Technology Invention Award in 2015, the first prize of the CIE Scientific and Technological Progress Award in 2022, and the special grand prize of Guangdong Technology Progress award in 2023.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/xiangyuan_lan.jpg}}]{Xiangyuan Lan} received a B.Eng. degree from the South China University of Technology, China, in 2012, and the Ph.D. degree from Hong Kong Baptist University, Hong Kong, in 2016. He was a Visiting Scholar with the University of Maryland, College Park, MD, USA, in 2015, and also a Visiting Researcher with the University of California at Merced, Merced, CA, USA, in 2017. He was a Post-Doctoral Research Fellow from 2016 to 2018 and then a Research Assistant Professor from 2018 to 2021, with Hong Kong Baptist University. He joined the Peng Cheng Laboratory, Shenzhen, China, in 2022, where he is currently an Associate Professor. He is a Ph.D. Supervisor affiliated with the Southern University of Science and Technology, China, and an external supervisor at Tsinghua University. He is currently an Associate Editor of Signal, Image, and Video Processing and Frontiers in Signal Processing. His current research interests include pre-trained foundation models and their applications in multi-modal perception.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/xiaodan_liang.jpg}}]{Xiaodan Liang} is currently an Associate Professor at Sun Yat-sen University. She was a postdoc researcher in the machine learning department at Carnegie Mellon University, working with Prof. Eric Xing, from 2016 to 2018. She received her Ph.D. degree from Sun Yat-sen University in 2016. She has published several cutting-edge projects on human-related analysis, including human parsing, pedestrian detection, instance segmentation, 2D/3D human pose estimation, and activity recognition.
\end{IEEEbiography}

\vspace{11pt}
\vfill
